Real-Time Safety Evaluation of Human Arm Operations Using a Wrist-Mounted IMU with PSM System

This paper presents a novel approach to real-time safety monitoring in human-robot collaborative manufacturing environments through a wrist-mounted Inertial Measurement Unit (IMU) system integrated with a Predictive Safety Model (PSM). The proposed system extends previous PSM implementations through the adaptation of a spring-damper-mass model specifically optimized for wrist motions, employing probabilistic safety assessment through impedance-based computations. We analyze our proposed impedance-based safety approach with frequency domain methods, establishing quantitative safety thresholds through comprehensive comparative analysis. Experimental validation across three manufacturing tasks - tool manipulation, visual inspection, and pick-and-place operations. Results show robust performance across diverse manufacturing scenarios while maintaining computational efficiency through optimized parameter selection. This work establishes a foundation for future developments in adaptive risk assessment in real-time for human-robot collaborative manufacturing environments.

==> EXTRA.tex <==
% This part is temporary as notes for you
% It looks like we 
The rolling disk with angle $\varphi_ir$ with rotating pendulum angle $\theta_i$ for the angular states of $\bm{q}=[\varphi_i,\theta_i]$ is defined as 
\begin{align}
\uvec{M}(\bm{q})\bm{\ddot{q}}+\uvec{h}(\bm{q},\bm{\dot{q}})=\uvec{u},
\label{Eq:MotionEquationGeneral}
%\label{Eq:motionmechanismsystem}
\end{align}
where inertial matrix $\uvec{M}(\bm{q})$, velocity dependencies $N_i$ and gravity terms $G_i$ in $\uvec{h}(\bm{q},\bm{\dot{q}})$ and control inputs $\uvec{u}$ are defined by \cite{tafrishi2020singularity}
\begin{align*}{\small
\uvec{M}(\bm{q})= \left[\begin{array}{cc} M_{11}\;  M_{12}\\ M_{21}\; M_{22}\\ \end{array}\right],\uvec{h}(\bm{q},\bm{\dot{q}})= \left[\begin{array}{c}N_1+G_1\\ G_2\\ \end{array}\right],\uvec{u}=\left[\begin{array}{c}0\\ \tau_{\varphi}\\ \end{array}\right].}
\end{align*}
where the parameters are found as 
\begin{align}
\begin{split}
&M_{11}=I_p+M R^2+I_d+m R^2-2m R r \cos(\varphi+\theta) + m r^2, \\
&M_{12}=M_{21}=I_p -m R r \cos(\varphi+\theta)+ m r^2,M_{22}=I_p+ m r^2,\\
&N_{1}=m R r(\dot\varphi+\dot\theta)^2 \sin(\varphi+\theta), G_{1}= G_{2}=m   g r \sin(\varphi+\theta).
\end{split}
\label{Eq:NONLINEARDynamics} 
\end{align}
To check the stability of the model, we linearized the rolling pendulum-actuated disk around lower zero equilibrium which resulted in having our state-space model for each disk as 
\begin{align}
    \uvec{A}= \left[\begin{array}{cccc} M_{11} & & & M_{12}\\ M_{21}& & & M_{22}\\
    & & & \\
    & & & \end{array}\right]  , \uvec{B}=  \uvec{C} , \uvec{D} 
\end{align}
